Free Foil: Generating Efficient and Scope-Safe Abstract Syntax

Handling bound identifiers correctly and efficiently is critical in implementations of compilers, proof assistants, and theorem provers. When choosing a representation for abstract syntax with binders, implementors face a trade-off between type safety with intrinsic scoping, efficiency, and generality. The "foil" by Maclaurin, Radul, and Paszke combines an efficient implementation of the Barendregt convention with intrinsic scoping through advanced type system features in Haskell, such as rank-2 polymorphism and generalized algebraic data types. Free scoped monads of Kudasov, on the other hand, combine intrinsic scoping with de Bruijn indices as nested data types with Sweirstra's data types \`a la carte approach to allow generic implementation of algorithms such as higher-order unification. In this paper, we suggest two approaches of making the foil more affordable. First, we marry free scoped monads with the foil, allowing to generate efficient, type-safe, and generic abstract syntax representation with binders for any language given its second-order signature. Second, we provide Template Haskell functions that allow generating the scope-safe representation from a na\"ive one. The latter approach enables us to use existing tools like BNF Converter to very quickly prototype complete implementation of languages, including parsing, pretty-printing, and efficient intrinsically scoped abstract syntax. We demonstrate both approaches using $\lambda\Pi$ with pairs and patterns as our example object language. Finally, we provide benchmarks comparing our implementation against the foil, free scoped monads with nested de Bruijn indices, and some traditional implementations.

==> sections/5-example.tex <==
\section{Example: implementing $\lambda\Pi$}
\label{section:example}

In this section, we demonstrate two ways to implement $\lambda\Pi$.
First, we show how to generate the syntax and substitution from a signature.
Second, we show how to use extention to get also parser, pretty-printer, 
and other utilities. We will then show how to implement typechecking for $\lambda\Pi$-terms
using the generated syntax and highlighting the safety features arising from using the Foil.

\subsection{Generating syntax from a signature}


\subsection{Generating syntax using Template Haskell}

\begin{figure}
  \begin{minted}{ebnf}
    comment "--" ;
    comment "{-" "-}" ;

    layout toplevel ;

    token VarIdent letter (letter | digit | '_' | '\'')* ;

    AProgram. Program ::= [Command] ;

    CommandCheck.   Command ::= "check"   Term ":" Term ;
    CommandCompute. Command ::= "compute" Term ":" Term ;
    terminator Command ";" ;

    Lam.  Term ::= "λ" Pattern "." ScopedTerm ;
    Pi.   Term ::= "Π" "(" Pattern ":" Term ")" "→" ScopedTerm ;
    App.  Term1 ::= Term1 Term2 ;
    Var.  Term2 ::= VarIdent ;
    coercions Term 2 ;

    AScopedTerm. ScopedTerm ::= Term ;

    PatternVar.     Pattern ::= VarIdent ;
    PatternPair.    Pattern ::= VarIdent VarIdent ;
    PatternTriplet. Pattern ::= VarIdent VarIdent VarIdent ;    
  \end{minted}
  \label{figure:lambda-pi-scoped-bnfc}
  \caption{BNF with scope annotations for $\lambda\Pi$.}
\end{figure}

First we need to decide on the grammar of the language. We will use the grammar presented in /ref{figure:lambda-pi-scoped-bnfc}.
We show this particular grammar as an example because it is able to show the constructions we need. 
In particular:
\begin{itemize}
  \item The Lam and Pi rules show the places where the Scope of the program is extended by one or more new variables
  \item Pattern** denote the new variables declaration (binders).
  \item AScopedTerm denotes the location where new variables will be available in the program Scope.
\end{itemize}

Once the grammar is defined, the build process follows. During this moment, the 
BNFC solution (BNF-converter) generates the necessary data structures/ref{figure:lambda-pi-signature}.
In this article we will present only these data structures, as they are the most important, 
unlike the Skeleton and Pretty-Printer implementations. Here we can observe that all the constructs remain unchanged, 
as well as their names.

\begin{figure}
  \begin{minted}{haskell}
    data Term
        = Lam Pattern ScopedTerm
        | Pi Pattern Term ScopedTerm
        | App Term Term
        | Var VarIdent

    data ScopedTerm = AScopedTerm Term

    data Pattern
        = PatternVar VarIdent
        | PatternPair VarIdent VarIdent
        | PatternTriplet VarIdent VarIdent VarIdent
  \end{minted}
  \label{figure:lambda-pi-signature}
  \caption{Signature for $\lambda\Pi$ in Haskell.}
\end{figure}

Then from the grammar provided by BNFC we generate a Scope-safe grammar using 4 simple lines of code\ref{figure:foil-lambda-pi-generation}. 

\begin{figure}
  \begin{minted}{haskell}
    mkFoilData ''Term ''VarIdent ''ScopedTerm ''Pattern
    mkToFoil ''Term ''VarIdent ''ScopedTerm ''Pattern
    mkFromFoil ''Term ''VarIdent ''ScopedTerm ''Pattern
    mkInstancesFoil ''Term ''VarIdent ''ScopedTerm ''Pattern
  \end{minted}
  \label{figure:foil-lambda-pi-generation}
  \caption{Signature for Foil $\lambda\Pi$ in Haskell.}
\end{figure}

Finally we can see the generated Scope-safe grammar\ref{figure:foil-lambda-pi-signature}.
This example shows, among other things, the safety of working with Scopes. To notice it, 
you should pay attention to the kinds that will help you avoid mistakes when working with the language.

\begin{figure}
  \begin{minted}{haskell}
    data FoilTerm n where
        FoilLam :: FoilPattern n t1 t2 l -> FoilScopedTerm l -> FoilTerm n
        FoilPi :: FoilPattern n t1 t2 l -> FoilTerm n -> FoilScopedTerm l -> FoilTerm n
        FoilApp :: FoilTerm n -> FoilTerm n -> FoilTerm n
        FoilVar :: Name n -> FoilTerm n
    
    data FoilPattern n t1 t2 l
      = FoilPatternVar (NameBinder n l)
      | FoilPatternPair (NameBinder n t1) (NameBinder t1 l)
      | FoilPatternTriplet (NameBinder n t1) (NameBinder t1 t2) (NameBinder t2 l)
    
    data FoilScopedTerm n
      = FoilAScopedTerm (FoilTerm n)

  \end{minted}
  \label{figure:foil-lambda-pi-signature}
  \caption{Signature for Foil $\lambda\Pi$ in Haskell.}
\end{figure}

\subsection{Typechecking $\lambda\Pi$ terms}

\nikolai{To be done.}


==> sections/7-haskell-vs-scala.tex <==
\section{Haskell versus Scala}
\label{section:haskell-vs-scala}


Haskell offers a wide range of advanced features and powerful abstractions. As a result, when porting code from Haskell to Scala, it may be necessary to adapt certain Haskell-specific features to achieve the same level of expressiveness and functionality.

One such feature is higher-rank polymorphism, which allows functions to take or return polymorphic functions as arguments. In Haskell, higher-rank polymorphism enables the creation of highly abstract and reusable code. However, Scala's type system is not as expressive when it comes to higher-rank polymorphism, requiring some adaptation and alternative approaches to achieve similar results.

Another feature is partial application of types. In Haskell, it is possible to partially apply type constructors, allowing for more flexible and reusable type definitions.

Partial application of types enables the creation of higher-order types, where type constructors are treated as first-class entities. This allows for the easy creation of generic types that can represent a wide range of specific types.

In Scala, partial application of types is not directly supported in the same way as in Haskell. However, Scala provides alternatives such as type lambdas \cite{type-lambdas} and higher-kinded types \cite{scalaHKD} that can achieve similar results.

Type lambdas allow the creation of anonymous type functions, which take types as input parameters and produce new types as output.

Higher-kinded types, also known as higher-kinded polymorphism, provide a mechanism for abstracting over type constructors. They allow for the definition of generic type constructors that can be partially applied or combined with other type constructors to create new types.

Because Scala 3 offers more powerful and convenient syntax constructs than Scala 2, as well as improved type support and language features, we decided to use Scala 3.

In the following sections we show how to rewrite some code snippets from Haskell to Scala.

\subsection{Rank-2 polymorphism}

The Foil use rank-2 polymorphism in function definitions. In particular,

\begin{minted}{haskell}
    withFreshBinder :: Scope n -> (forall l. NameBindernl -> r) -> r
    withFreshBinder (UnsafeScope rs) cont = cont binder where
      binder =UnsafeBinder (UnsafeName(rawFreshNamers))
\end{minted}

The rank-2 polymorphism is the language extension in Haskell and does not supported in Scala 2 out of the box. Scala 3 has new features named Polymorphic function types \cite{polymorphic-function-types}. This feature provides the ability to describe and use functions that are polymorphic with respect to types.

Function definition with rank-2 polymorphism with Scala 3 will look like:

\begin{minted}{scala}
    def withFreshBinder[N <: S, R](
     scope: Scope[N],
     cont: [L <: S] => NameBinder[N, L] => R
    ): R =
    cont(NameBinder(Name(rawFreshName(scope.unsafeScope))))
\end{minted}

However, in Scala 2 the similar behaviour still can be achieved using FuntionK \cite{functionK} from Cats library.

 \subsection{Partial applied types}

In Free Foil we have following data types:
\begin{minted}{haskell}
    data ScopedAST sig n where
      ScopedAST :: Foil.NameBinder n l -> AST sig l -> ScopedAST sig n

    data AST sig n where
      Var :: Foil.Name n -> AST sig n
      Node :: sig (ScopedAST sig n) (AST sig n) -> AST sig n
\end{minted}

 For that data types we need to instantiate \haskell{Foil.Substitution (AST sig) i o}, where \haskell{Substitution} has the following signature:

 \begin{minted}{haskell}
    data Substitution (e:: S -> *) (i:: S) (o :: S) =
      UnsafeSubstitution (forall n. Name n -> e n) (IM.IntMap (e o))
 \end{minted}

 In Scala \haskell{Substitution} and another types from above can be denoted as:
 \begin{minted}{scala}
    case class ScopedAST[Sig[_, _], N <: S, L <: S](
      binder: Foil.NameBinder[N, L], ast: AST[Sig, L]
    )

    sealed trait AST[Sig[_, _], N <: S]
    case class Var[Sig[_, _], N <: S](name: Foil.Name[N])  extends AST[Sig, N]
    case class Node[Sig[_, _], N <: S, L <: S](
      sig: Sig[ScopedAST[Sig, N, L], AST[Sig, N]]
    ) extends AST[Sig, N]

    case class Substitution[E[_ <: S], I <: S, O <: S](
      f: [N <: S] => Name[N] => E[N],
      env: IntMap[E[O]]
    )
 \end{minted}

 To correct instantiation \haskell{Substitution} with \haskell{AST} as the first type parameter needs the partial type application. Because such features is not supported in Scala, the correct implementation using type lambdas is:

 \begin{minted}{scala}
     subst: Substitution[[Y <: S] =>> AST[Sig, Y], I, O]
 \end{minted}
 \subsection{Bifunctors}

 \subsection{Pattern Synonyms}

